TEEMATE: Fast and Efficient Confidential Container using Shared Enclave

Confidential container is becoming increasingly popular as it meets both needs for efficient resource management by cloud providers, and data protection by cloud users. Specifically, confidential containers integrate the container and the enclave, aiming to inherit the design-wise advantages of both (i.e., resource management and data protection). However, current confidential containers suffer from large performance overheads caused by i) a larger startup latency due to the enclave creation, and ii) a larger memory footprint due to the non-shareable characteristics of enclave memory. This paper explores a design conundrum of confidential container, examining why the confidential containers impose such large performance overheads. Surprisingly, we found there is a universal misconception that an enclave can only be used by a single (containerized) process that created it. However, an enclave can be shared across multiple processes, because an enclave is merely a set of physical resources while the process is an abstraction constructed by the host kernel. To this end, we introduce TeeMate, a new approach to utilize the enclaves on the host system. Especially, TeeMate designs the primitives to i) share the enclave memory between processes, thus preserving memory abstraction, and ii) assign the threads in enclave between processes, thus preserving thread abstraction. We concretized TeeMate on Intel SGX, and implemented confidential serverless computing and confidential database on top of TeeMate based confidential containers. The evaluation clearly demonstrated the strong practical impact of TeeMate by achieving at least 4.5 times lower latency and 2.8 times lower memory usage compared to the applications built on the conventional confidential containers.

==> Makefile <==
MAIN ?= p
DIFF ?= HEAD^
CODE := $(addsuffix .tex,$(filter-out %.tex,$(wildcard code/*)))
FIGS := $(patsubst %.svg,%.pdf,$(wildcard fig/*.svg))
ODGS := $(patsubst %.odg,%.pdf,$(wildcard fig/*.odg))
PLOT := $(patsubst %.gp,%.tex,$(wildcard data/*.gp))
DEPS := rev.tex code/fmt.tex abstract.txt $(CODE) $(FIGS) $(ODGS) $(PLOT)
LTEX := --latex-args="-synctex=1 -shell-escape"
BTEX := --bibtex-args="-min-crossrefs=99"
SHELL:= $(shell echo $$SHELL)

all: $(DEPS) ## generate a pdf
	@TEXINPUTS="sty:" bin/latexrun $(LTEX) $(BTEX) $(MAIN)
	cp latex.out/$(MAIN).synctex.gz .

submit: $(DEPS) ## proposal function
	@for f in $(wildcard submit-*.tex); do \
		TEXINPUTS="sty:" bin/latexrun $$f; \
	done

diff: $(DEPS) ## generate diff-highlighed pdf
	@bin/diff.sh $(DIFF)

help: ## print help
	@grep -E '^[a-zA-Z_-]+:.*?## .*$$' $(MAKEFILE_LIST) \
	  | sort | awk 'BEGIN {FS = ":.*?## "}; {printf "\033[36m%-10s\033[0m %s\n", $$1, $$2}'

rev.tex: FORCE
	@printf '\\gdef\\therev{%s}\n\\gdef\\thedate{%s}\n' \
	   "$(shell git rev-parse --short HEAD)"            \
	   "$(shell git log -1 --format='%ci' HEAD)" > $@

code/%.tex: code/% ## build highlighted tex code from source code
	pygmentize -P tabsize=4 -P mathescape -f latex $^ | bin/mark.py > $@

code/fmt.tex: ## generate color table
	pygmentize -f latex -S default > $@

fig/%.pdf: fig/%.svg ## generate pdf from svg
	bin/svg2pdf.sh ${CURDIR}/$^ ${CURDIR}/$@

fig/%.pdf: fig/%.odg ## generate pdf from LibreOffice Draw
	bin/odg2pdf.sh $^ $@

data/%.tex: data/%.gp ## generate plot
	gnuplot $^

data/%.pdf: data/%.py ## generate plot
	python3 $^

draft: $(DEPS) ## generate pdf with a draft info
	echo -e '\\newcommand*{\\DRAFT}{}' >> rev.tex
	@TEXINPUTS="sty:" bin/latexrun $(BTEX) $(MAIN)

watermark: $(DEPS) ## generate pdf with a watermark
	echo -e '\\usepackage[firstpage]{draftwatermark}' >> rev.tex
	@TEXINPUTS="sty:" bin/latexrun $(BTEX) $(MAIN)

spell: ## run a spell check
	@for i in *.tex; do bin/aspell.sh tex $$i; done
	@for i in *.tex; do bin/double.pl $$i; done
	@for i in *.tex; do bin/abbrv.pl  $$i; done
	@bin/hyphens.sh *.tex
	@pdftotext $(MAIN).pdf /dev/stdout | grep '??'
	@for i in fig/*.svg; do bin/aspell.sh svg $$i; done
	@for i in code/*.c; do bin/aspell.sh code $$i; done

bib: all ## print bib used in the paper
	bibexport latex.out/$(MAIN).aux

clean: ## clean up
	@bin/latexrun --clean
	rm -f abstract.txt
	rm -f $(MAIN).synctex.gz

distclean: clean ## clean up completely
	rm -f code/*.tex
	rm -rf _minted_p

abstract.txt: abstract.tex $(MAIN).tex ## generate abstract.txt
	@bin/mkabstract $(MAIN).tex $< | fmt -w72 > $@

.PHONY: all help FORCE draft clean spell distclean init bib


==> README <==
die: a paper template
=====================

## start

0. Prerequisites

  - Python 3.x
  - pygmentize

    $ pip install Pygments 

1. clone the git repo:

  - if you have none,

    $ git clone --depth=1 git@github.com:tsgates/die.git

  - if you have a git-repo to work on,

    $ git subtree add --squash git@github.com:tsgates/die.git master -P paper

  - or

    $ wget https://github.com/tsgates/die/releases/download/latest/die.tar.gz

2. build it:

    $ make
    p.pdf built @Tue May 20 20:38:19 EDT 2014
    
    (check p.pdf)

3. starting point, p.tex:

    $ grep -oP 'input{\K\w+' p.tex
    cmds
    rev
   *hdr
    abstract
   *ex
    intro
    overview
    design
    impl
    eval
    conclusion
    ack

  - hdr: includes title/author info
  - ex : includes latex examples

4. example latex

    $ git checkout example
    $ make

5. formatting rules (dependencies)

  - code/*.{c,cc,py,js ...} -> code/*.tex
  - fig/*.svg               -> fig/*.pdf
  - data/*.gp               -> fig/*.tex

  (see ex.tex for more details)

## tools

1. make a draft for revision

    $ make draft
    $ make watermark

2. abstract.txt (from abstract.tex)

    $ cat abstract.txt 

3. highlight changes, since the last submit

    $ make diff DIFF=HEAD@{}

4. spell check

    $ make spell

## Acknowledgment

This template contains a few files copied/stolen from the Internet and
mainly from my past collaborators (e.g., sty/*, conf.bib, some bin/),
which I couldn't keep track of their licenses.

==> ack.tex <==
\section{Acknowledgment}
\label{s:ack}


==> app.tex <==
\section{Applications}
\label{s:app}



\subsection{Confidential Serverless Computing}
\label{ss:app-serverless}

\subsubsection{Implementation of In-enclave Isolation}
\label{sss:app-serverless-isolation}

\subsection{Confidential Database}
\label{ss:app-database}

\subsubsection{Implementation of In-enclave Isolation}
\label{sss:app-database-isolation}


==> background.tex <==
\section{Confidential Container}
\label{s:background}
In this section, we provide a brief background to understand the confidential
container, a secure container that leverages confidential computing.
First, we describe container~(\autoref{ss:back-container}), and then we explain
Intel SGX, which is a confidential computing technique suitable for confidential
container~(\autoref{ss:back-confidential-computing}).
Lastly, we illustrate the the design of confidential container, based on
comparison between regular container~(\autoref{ss:back-confidential-container}).

\subsection{Container}
\label{ss:back-container}
Container has gained popularity as a resource management unit in recent cloud
computing. 
Cloud providers have become responsible for resource management in models like
function-as-a-service (FaaS)~\cite{} or software-as-a-service (SaaS)~\cite{}. 
Container is well-suited for these models because they offer built-in resource
management mechanisms and efficient isolation to cloud providers.
By utilizing kernel features like cgroup~\cite{} and namespace~\cite{}, cloud
providers can easily track the hardware resource usage of each container.
This capability enables precise billing and performance isolation enforcement by
the cloud providers.
Additionally, containers provide a lightweight virtualization by encapsulating
only the application code and its dependencies, rather than the entire operating
system.
This results in lower memory consumption compared to virtual machine, allowing
cloud providers to maximize resource utilization.

\subsection{Intel SGX}
\label{ss:back-confidential-computing}
Intel Software Guard Extensions (SGX)~\cite{anati2013innovative} is a
confidential computing technique, which provides enclave for user-level
applications. 
SGX enclave is a protected physical memory region composed of EPC (Enclave Page
Cache) pages.
These EPC pages cannot be directly accessed or modified by system components
including hypervisors and operating systems.
This guarantees the confidentiality and integrity of the application data and
code inside enclave.
In addition, SGX enclave provides measurement and attestation
services~\cite{sgx-remote-attest}, with which enclave owner can check the
initial state of the enclave including the code and data, thereby ensuring its
initial integrity.

Intel SGX is a well-suited confidential computing technique in the scenario
where cloud providers use container for resource management.
Intel SGX differs from other confidential computing techniques~\cite{}, in
that it only encapsulates the user-level application, rather than the entire
operating system. 
This allows application to be protected against system software using enclave,
while cloud providers can fully utilize kernel features for resource management.

In this paper, we focus on the confidential container that utilizes Intel SGX,
since Intel SGX can be integrated well to container as mentioned above.
However, we emphasize that our motivation and key idea can be applied to other
confidential computing technologies as we will mention in \autoref{s:discuss}.

\begin{figure}[t]
  \centering
  \begin{subfigure}{0.48\columnwidth}
    \includegraphics[width=\linewidth]{fig/motiv/motiv-Container-1.pdf}
    \caption{Virtual \& Physical address space}
    \label{fig:motiv-container-vapa}
  \end{subfigure}
  \hspace{5pt}
  \begin{subfigure}{0.42\columnwidth}
    \vspace{8pt}
    \includegraphics[width=\linewidth]{fig/motiv/motiv-Container-2.pdf}
    \caption{Software stack}
    \label{fig:motiv-container-software-stack}
  \end{subfigure}
  \caption{Comparison between regular and confidential container}
  \label{fig:motiv-container}
\end{figure}
\subsection{Confidential Container vs Regular Container}
\label{ss:back-confidential-container}
As shown in~\autoref{fig:motiv-container-vapa}, the main distinction of a
confidential container compared to a regular container is that it leverages an
enclave.
Specifically, a process inside the confidential container maps its virtual
address range to the enclave's physical address range.
The enclave is composed of multiple EPC pages, which are protected physical
memory pages by SGX hardware. 
Confidential container can load and run the application inside the enclave so
that it can be protected against the untrusted components outside the enclave.

Confidential container also has a slightly different software stack compared to
a regular container as illustrated
in~\autoref{fig:motiv-container-software-stack}.
A regular container first loads a runtime and then loads and executes an
application on top of it.
On the other hand, a confidential container first loads an enclave runtime,
which provides compatible abstraction layers for an enclave environment, inside
enclave.
This includes either a library OS (e.g., Gramine~\cite{tsai2017graphene},
SGX-LKL~\cite{priebe2019sgxlkl}, Haven~\cite{Baumann2014haven}) or a simple
shim-layer (e.g., Scone~\cite{arnautov2016scone},
Panoply~\cite{shinde2017panoply}).
After that, the confidential container loads and executes runtime and
application on top of the enclave runtime, which is largely same as the regular
container.





































































==> code/fmt.tex <==

\makeatletter
\def\PY@reset{\let\PY@it=\relax \let\PY@bf=\relax%
    \let\PY@ul=\relax \let\PY@tc=\relax%
    \let\PY@bc=\relax \let\PY@ff=\relax}
\def\PY@tok#1{\csname PY@tok@#1\endcsname}
\def\PY@toks#1+{\ifx\relax#1\empty\else%
    \PY@tok{#1}\expandafter\PY@toks\fi}
\def\PY@do#1{\PY@bc{\PY@tc{\PY@ul{%
    \PY@it{\PY@bf{\PY@ff{#1}}}}}}}
\def\PY#1#2{\PY@reset\PY@toks#1+\relax+\PY@do{#2}}

\@namedef{PY@tok@w}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\@namedef{PY@tok@c}{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.24,0.48,0.48}{##1}}}
\@namedef{PY@tok@cp}{\def\PY@tc##1{\textcolor[rgb]{0.61,0.40,0.00}{##1}}}
\@namedef{PY@tok@k}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@kp}{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@kt}{\def\PY@tc##1{\textcolor[rgb]{0.69,0.00,0.25}{##1}}}
\@namedef{PY@tok@o}{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PY@tok@ow}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\@namedef{PY@tok@nb}{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@nf}{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\@namedef{PY@tok@nc}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\@namedef{PY@tok@nn}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\@namedef{PY@tok@ne}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.80,0.25,0.22}{##1}}}
\@namedef{PY@tok@nv}{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\@namedef{PY@tok@no}{\def\PY@tc##1{\textcolor[rgb]{0.53,0.00,0.00}{##1}}}
\@namedef{PY@tok@nl}{\def\PY@tc##1{\textcolor[rgb]{0.46,0.46,0.00}{##1}}}
\@namedef{PY@tok@ni}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.44,0.44,0.44}{##1}}}
\@namedef{PY@tok@na}{\def\PY@tc##1{\textcolor[rgb]{0.41,0.47,0.13}{##1}}}
\@namedef{PY@tok@nt}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@nd}{\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\@namedef{PY@tok@s}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@sd}{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@si}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.64,0.35,0.47}{##1}}}
\@namedef{PY@tok@se}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.36,0.12}{##1}}}
\@namedef{PY@tok@sr}{\def\PY@tc##1{\textcolor[rgb]{0.64,0.35,0.47}{##1}}}
\@namedef{PY@tok@ss}{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\@namedef{PY@tok@sx}{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@m}{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PY@tok@gh}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\@namedef{PY@tok@gu}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\@namedef{PY@tok@gd}{\def\PY@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\@namedef{PY@tok@gi}{\def\PY@tc##1{\textcolor[rgb]{0.00,0.52,0.00}{##1}}}
\@namedef{PY@tok@gr}{\def\PY@tc##1{\textcolor[rgb]{0.89,0.00,0.00}{##1}}}
\@namedef{PY@tok@ge}{\let\PY@it=\textit}
\@namedef{PY@tok@gs}{\let\PY@bf=\textbf}
\@namedef{PY@tok@ges}{\let\PY@bf=\textbf\let\PY@it=\textit}
\@namedef{PY@tok@gp}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\@namedef{PY@tok@go}{\def\PY@tc##1{\textcolor[rgb]{0.44,0.44,0.44}{##1}}}
\@namedef{PY@tok@gt}{\def\PY@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\@namedef{PY@tok@err}{\def\PY@bc##1{{\setlength{\fboxsep}{\string -\fboxrule}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}}
\@namedef{PY@tok@kc}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@kd}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@kn}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@kr}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@bp}{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@fm}{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\@namedef{PY@tok@vc}{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\@namedef{PY@tok@vg}{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\@namedef{PY@tok@vi}{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\@namedef{PY@tok@vm}{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\@namedef{PY@tok@sa}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@sb}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@sc}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@dl}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@s2}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@sh}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@s1}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@mb}{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PY@tok@mf}{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PY@tok@mh}{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PY@tok@mi}{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PY@tok@il}{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PY@tok@mo}{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PY@tok@ch}{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.24,0.48,0.48}{##1}}}
\@namedef{PY@tok@cm}{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.24,0.48,0.48}{##1}}}
\@namedef{PY@tok@cpf}{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.24,0.48,0.48}{##1}}}
\@namedef{PY@tok@c1}{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.24,0.48,0.48}{##1}}}
\@namedef{PY@tok@cs}{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.24,0.48,0.48}{##1}}}

\def\PYZbs{\char`\\}
\def\PYZus{\char`\_}
\def\PYZob{\char`\{}
\def\PYZcb{\char`\}}
\def\PYZca{\char`\^}
\def\PYZam{\char`\&}
\def\PYZlt{\char`\<}
\def\PYZgt{\char`\>}
\def\PYZsh{\char`\#}
\def\PYZpc{\char`\%}
\def\PYZdl{\char`\$}
\def\PYZhy{\char`\-}
\def\PYZsq{\char`\'}
\def\PYZdq{\char`\"}
\def\PYZti{\char`\~}
\def\PYZat{@}
\def\PYZlb{[}
\def\PYZrb{]}
\makeatother



==> design2.tex <==
\section{Primitive Design Features of \sys}
\label{s:design}


In order to address performance limitations of confidential serverless
computing, \sys develops two primitive design features leveraging
unique features of Intel SGX~\cite{costan2016intel}:
(i) \enclaveAliasing, which allows \sys to share EPC pages across
multiple containers~(\autoref{ss:design-sharing});
and (ii) container-independent enclave threads, which enables \sys to
execute container-independent enclave
threads~(\autoref{ss:design-execution-context}).
As we will describe later in~\autoref{s:design2}, these two primitive
features will be used together to construct an efficient confidential
serverless framework.



\subsection{Sharing Enclave Pages across Containers}
\label{ss:design-sharing}

\enclaveAliasing is a new technique, allowing to share a single SGX
enclave across multiple processes.
In the following, we first explain the address translation and
validation mechanism of SGX, particularly for EPC pages.
Then we illustrate how \sys leverages such a mechanism to enable
\enclaveAliasing.


\PP{Technical Analysis: Address Translation and Validation in SGX}
SGX ensures the integrity of the virtual-to-physical address mapping
for EPC pages, preventing malicious system components from launching
a page remapping attack (e.g., tricking a victim enclave to access a
different EPC page through the same virtual address~\cite{costan2016intel}).
This integrity is assured by maintaining additional address mapping
within the special EPC page, so called EPCM.
Specifically, when a new EPC page is allocated, the kernel updates the
page table with virtual-to-physical address mapping (e.g., \cc{VA} to
\cc{PA}) related to the EPC page.
When the kernel requests the CPU to create the EPC pages, the CPU
creates a new EPCM entry per new EPC page, which contains \cc{VA} of
the corresponding EPC page located at \cc{PA}.
When any access to the EPC page is attempted later using \cc{VA}, the
CPU translates \cc{VA} to \cc{PA} using the page table.
However, since the page table can be compromised by the adversarial
systems components, the CPU further validates that such a translation
is correct using EPCM, thereby assuring the integrity of the
virtual-to-physical address mapping.

An interesting technical characteristic here is in the
address validation mechanism of EPCM, which does not involve
the identity of a process (i.e., EPCM does not include
process identifiers like ASID~\cite{armv7a}).
Thus, an EPC page (located at \cc{PA}) can be accessed by any
other processes using \cc{VA} as long as the page table of
the process contains the same mapping from \cc{VA} to
\cc{PA}.
If so, the process, which did not initially create the EPC page, can
still access the EPC page through accessing to the same \cc{VA}.
Note that while this may seem a vulnerable design, it does not harm
the security assurance of SGX, which we elaborate the detailed
security analysis in~\autoref{s:security-analysis}.



\begin{figure}[t]
  \centering
  \includegraphics[width=0.7\linewidth]{fig/design/VACondition.pdf}
  \caption{Sharing the same EPC pages across different containers
    using \enclaveAliasing}
\label{fig:design-VACondition}
\vspace{-10pt}
\end{figure}


\PP{EPC Aliasing}
To alias EPC pages across different processes, \sys leverages
previously mentioned EPCM's characteristics.
Specifically, \enclaveAliasing maps multiple virtual pages to the same
physical EPC page, where multiple virtual pages are (i) associated
with different processes and (ii) these virtual pages have the same
virtual address.
More technically, if a process $\cc{p}_0$ already allocated an EPC
page with address mapping (i.e., \VAzero to \PAzero), \enclaveAliasing
allows to map the same EPC page to another process $\cc{p}_1$ by
updating $\cc{p}_1$'s page table, inserting \VAzero to \PAzero address
mapping.
After that, the process $\cc{p}_1$ can also access the EPC page
with virtual address \VAzero.

In order to share EPC pages between containers, \sys performs the
\enclaveAliasing as illustrated in~\autoref{fig:design-VACondition}.
Specifically, \sys creates the initial container.
Then, after identifying available virtual and physical pages for an
enclave, the kernel updates the page table of the initial container
---i.e., adding an address mapping from \VAzero and \VAone to
\PAzero and \PAone, respectively~(\WC{1}).
Then the kernel requests the CPU to allocate new physical EPC pages
using the SGX instruction (i.e., \cc{EADD}~\cite{costan2016intel})
(\WC{2}).
This consequently makes CPU to create an EPCM entry corresponding to
\PAzero and \PAone, which contains \VAzero and \VAone, respectively~(\WC{3}).
At this point, in order to share and thus alias this EPC page later,
\sys additionally records the mappings for \VAzero and
\VAone~(\WC{4}).


When creating a new container, \sys aliases the previously allocated
EPC pages.
This entails to insert the recorded address mapping---i.e., (\VAzero,
\PAzero) and (\VAone, \PAone)---to the page table of the new
container~(\WC{5}).
Therefore, when the new container accesses the memory with \VAzero or
\VAone, the CPU would accordingly translate it to the aliased EPC page
located at \PAzero or \PAone using (i) the page table of the new
container and (ii) the corresponding EPCM entry.



From the performance perspective, EPC aliasing significantly reduces
the latency since it avoids to allocate redundant EPC pages as well as
loading a huge runtime (the steps from \WC{2} to \WC{4}
in~\autoref{sss:motiv-confidential}).
Furthermore, each new container only adds up minimal EPC pages
required for function instance (the step \WC{5}
in~\autoref{sss:motiv-confidential}) which needs much lower memory
than the previous confidential serverless approaches.



\subsection{Container-independent Enclave Threads}
\label{ss:design-execution-context}

Using \enclaveAliasing (\autoref{ss:design-sharing}), \sys
enables sharing enclave's EPC pages across multiple
containers.
Now this section presents how \sys enables individual execution
contexts across containers while sharing enclave's EPC pages.


\PP{Technical Analysis: Multi-threads in SGX Enclave}
In order to support parallelism, SGX designs unique schemes
for secure multi-threading within an enclave, which we refer
to as enclave threads~\cite{costan2016intel}.
In particular, the execution contexts of enclave threads are
managed by Thread Control Structures (TCSs), which are also
stored in the EPC pages to protect against adversarial
system components.
More technically, each TCS manages the entry point and the
CPU register context per enclave thread.
First, the entry point ensures that an enclave thread always
starts or resumes (i.e., \cc{EENTER} or \cc{ERESUME}) at the
code address designated in the given TCS (i.e., \cc{OENTRY}
field).
The entry point often contains security checks and
enforcement to sanitize the inputs from non-enclave
context.
Second, the CPU register context ensures that a paused
enclave thread is always resumed as expected.
This is carried out by saving (and restoring) all CPU
register values to (and from) the TCS\footnote{More
  precisely, TCS stores the reference to State Save Area
  (SSA) in the EPC pages.}, which happens when the enclave
thread exits (and resumes).
It is worth noting that initial TCS pages are measured as
other EPC pages, thereby preventing untrusted system components
from breaking its initial integrity.



The technical catch here is that unlike the typical use-cases of
multi-threading in SGX, we find that an enclave thread does not need
to be bound with a specific process.
In fact, an enclave thread can be migrated from one process to
another.
Specifically, when switching from the non-enclave execution context to
the enclave execution context, any TCS page can be selected and such a
selection does not restrict which process performs the switch (i.e.,
which process performs \cc{EENTER} or \cc{ERESUME}).
\sys leverages this operational property to enable individual
execution context per container while sharing the EPC memory pages.

\PP{Individual Enclave Thread per Container}
In order to support an enclave thread per container while aliasing EPC
pages, \sys designs management schemes to map between a TCS page and a
container.
As such, while sharing EPC pages, \sys assigns a dedicated
TCS page per enclave thread, where each enclave thread is
associated with a different containerized-process.


\begin{figure}[t]
  \centering
    \includegraphics[width=\linewidth]{fig/design/tcs-workflow-detail.pdf}
    \caption{Constructing container-independent enclave threads}
  \label{fig:design-TCS-workflow-order-old}
\end{figure}

More technically, \autoref{fig:design-TCS-workflow-order-old} shows
how \sys supports an individual enclave thread per container.
In this figure, we assume that a single container (i.e., $\cc{Container}_0$)
and an enclave were initially created before, where no enclave code has
been executed yet.
Accordingly, \sys initializes a TCS table, which indicates that all
TCS pages are available.
Next, a new container is created (i.e., $\cc{Container}_1$), which
shares the EPC pages through \enclaveAliasing.
To execute enclave threads per container, \sys first picks an
available TCS page per container (e.g., $\cc{tcs}_{0}$ for
$\cc{Container}_0$ and $\cc{tcs}_{1}$ for $\cc{Container}_1$,
respectively).
Then each container starts the execution of the enclave thread by
entering the enclave (i.e., \cc{EENTER}) with the chosen TCS
page.
Completing the execution of the enclave thread, the TCS table is
accordingly updated to mark which TCS page is now returned back to be
available.















\section{Applications}
\label{s:application}

Leveraging two design primitives presented in~\autoref{s:design}, now
we describe \sys-based confidential serverless computing, which
overcomes the performance limitation~(\autoref{ss:design2-workflow}).
Then we further describe how \sys mitigates the isolation issues
between function instances~(\autoref{ss:design2-isolation}).




\begin{figure}[t]
  \centering
  \begin{subfigure}{0.423\columnwidth}
    \includegraphics[width=\linewidth]{fig/design/overview-1.pdf}
    \caption{Application registration}
    \label{fig:design-overview-register}
    \vspace{15pt}
  \end{subfigure}
  \begin{subfigure}{0.457\columnwidth}
    \includegraphics[width=\linewidth]{fig/design/overview-2.pdf}
    \caption{Request handling}
    \label{fig:design-overview-handling}
    \vspace{15pt}
  \end{subfigure}
  \caption{Overall workflow and components of \sys.}
  \label{fig:design-overview}
\end{figure}


\subsection{Confidential Serverless Computing}
\label{ss:design2-workflow}

The overall workflow of \sys-based confidential serverless computing
is illustrated in~\autoref{fig:design-overview}, comprising two phases
that align with conventional serverless computing: (i) the application
registration phase and (ii) the request handling phase.

In the application registration phase (illustrated
in~\autoref{fig:design-overview-register}), the service provider
registers its own function code to \sys~(\WN{1}).
Once registered, \sys creates an initial container as well as an
enclave within the containerized-process.
Inside the enclave, \sys first loads \sys-runtime after accordingly
allocating new EPC pages~(\WN{2}).
Here, we denote \sys-runtime as the runtime including both
enclave-specific runtime and ordinary runtime for convenience.
At this point, no enclave code has been executed by far and thus \sys
performs the first-phase measurement, which is attested using the
original SGX's attestation mechanism~\cite{sgx-remote-attest}.
Right after the application registration phase, \sys controller
records the necessary enclave information for later use (\WN{3}).
This includes virtual-to-physical mapping for
\enclaveAliasing~(\autoref{ss:design-sharing}), and virtual address of
TCS pages to enable concurrent enclave threads per
container~(\autoref{ss:design-execution-context}).



The request handling phase (illustrated
in~\autoref{fig:design-overview-handling}) gets started as the
registered application receives the request from the clients~(\BC{1}).
There can be two different cases to determine the container to serve
the request:
(i) if the initial container is available, \sys reuses the initial
container to handle the request.
(ii) if the initial container is currently being used to serve other
request, \sys creates the new container~(\BC{2}) and then performs
\enclaveAliasing~(\BC{3}), which aliases EPC pages allocated for
\sys-runtime (as described in~\autoref{ss:design-sharing}).
After determining the container to handle the request, \sys selects
the available TCS page and initiates the execution of an enclave
thread using the selected TCS as described
in~\autoref{ss:design-execution-context}~(\BC{4}).
Once the enclave thread gets executed, \sys-runtime first loads the
function instance after allocating new EPC pages for those.
Then \sys-runtime hands the control over to the function instance,
which handles the client's request.
After handling the request, \sys-runtime deallocates EPC pages used
for the function instance.


\subsection{Isolation between Function Instances}
\label{ss:design2-isolation}

\begin{figure}[t]
  \centering
  \begin{subfigure}{0.4\columnwidth}
    \includegraphics[width=\linewidth]{fig/design/memory-isolation.pdf}
    \caption{Memory isolation}
    \label{fig:design-isolation-memory}
  \end{subfigure}
  \hspace{5pt}
  \begin{subfigure}{0.4\columnwidth}
    \includegraphics[width=\linewidth]{fig/design/fs-isolation.pdf}
    \caption{File system isolation}
    \label{fig:design-isolation-filesystem}
  \end{subfigure}
  \caption{Ensuring isolated context in the shared enclave}
  \label{fig:design-isolating}
\end{figure}


In \sys-based confidential serverless computing, the containers share the enclave memory
pages while executing with own enclave thread.
While this should be good for performances, this design alone do not
isolate function instances from each other, because all function
instances would be running within the same enclave.



To this end, \sys constructs its own isolation mechanisms as it cannot
rely on the isolation mechanisms of untrusted host kernel.
\sys performs the following isolation to secure resources:
i) prevent any memory accesses between the function instances and ii)
provide each function instance a unique userland view of global
resources (e.g., file systems and network stacks).


\PP{Memory Isolation}
In order to isolate the memory regions,
\sys leverages V8 Isolate~\cite{v8isolate} as shown
in~\autoref{fig:design-isolation-memory}.
To be specific, for each function instance, \sys-runtime
creates a V8 Isolate, which constructs an isolated memory
space (i.e., code, stack and heap).
The control and data flows are confined by the V8
Isolate, which ensures the function instances cannot access
each other's memory.
Additionally, we want to note that the isolation based on V8
Isolate is carefully designed as it supports most of popular
languages used in serverless
computing~\cite{nodejsispopular} (e.g., JavaScript in
native, and Python, Go, C, C++~\cite{c,cpp,go,python} through
WebAssembly~\cite{wasm}).


\PP{File System Isolation}
In order to isolate the file system, \sys provides an
in-memory file system while internally managing the file
mapping table as shown
in~\autoref{fig:design-isolation-filesystem}.
\sys handles every file operation from function instances
solely by the \sys-runtime in the enclave, not interacting
with outside file system.
Thus, untrusted host kernel cannot disturb with the file
system isolation of \sys-runtime.
In addition, \sys internally bookkeeps the files accessible
by each function instance through the file mapping table so
that the instances cannot read or write any file which
belongs to each another.



\PP{Handling Other Resources}
For the resources other than the file system (i.e., IPC,
UID, and network), we choose to simply disable or rely on
the host kernel.
For IPC and UID, \sys simply does not support the related
functionalities as they are not widely used in serverless
computing~\cite{nodejsispopular}.
For the network resources, \sys simply relies on host kernel
as it has to eventually receive the services from the
host kernel to access the network.
Meanwhile, the impact from a malicious kernel would be
minimized because the authentication and secure channel
construction are usually performed by the function instance
which runs in the enclave.
We want to note that \sys-runtime can be extended to support
isolating these resources also.









==> eval2.tex <==
\section{Evaluations on Applications}
\label{s:eval}

\subsection{Evaluation Setup}
\label{ss:eval-setup}

In this section, we evaluate various aspects of \sys.
We first describe the four serverless computing models
including \sys to be compared, and explain the evaluation
setup (\autoref{ss:eval-setup}).
Then, we evaluate the performance improvement of \sys in
terms of latency (\autoref{ss:eval-latency}), memory
efficiency (\autoref{ss:eval-memory}), and throughput
(\autoref{ss:eval-throughput}) respectively.
Finally, we showcase the performance of \sys in real-world
by simulating the client's requests
(\autoref{ss:eval-macro}).



\subsection{Evaluation Setup}
\label{ss:eval-setup}
\PP{Models for Comparison}
In order to clearly showcase the performance improvement of
\sys, we compare four models as summarized below:
\begin{itemize}[leftmargin=*]
  \setlength{\itemsep}{0.1pt}  
  \item \textbf{\modelNative} represents the conventional
        serverless computing, which does not use SGX enclave
        (i.e., \autoref{sss:motiv-serverless}).
  \item \textbf{\modelCcCold} is an existing approach to
        incorporate SGX enclave in serverless
        computing~\cite{li2021confidential,fritz2019sfaas,goltzsche2019acctee,trach2019clemmys},
        which creates a new enclave for every request as
        explained in~\autoref{sss:motiv-confidential}.
  \item \textbf{\modelCcWarm} is the same as the
        \modelCcCold model, while the only difference is
        that it pre-creates the execution environment (i.e.,
        container, SGX enclave, and function instance)
        before receiving the request.
        In this evaluation, we assume that 100\% of the
        requests can be predicted so that the environment is
        always prepared for incoming requests, except
        for~\autoref{ss:eval-macro}.
  \item \textbf{\sys} is our new model using
        \enclaveAliasing.
        It creates a initial container and an enclave in advance,
        and dynamically allocates new EPC pages only for function
        instances on demand.

\end{itemize}
We implemented all four models on OpenWhisk~\cite{openwhisk}
serverless platform.




\PP{Evaluation Environment}
We evaluated \sys and the other models on 64-core Intel Xeon
Gold 6348 CPU machine which supports SGX2 feature~\cite{xeon}.
Especially, we ran all the experiments in a QEMU virtual
machine~\cite{qemu} with 160GB memory and 48GB EPC size,
which runs a Linux kernel 6.2.0~\cite{linuxkernelv62}.
\begin{table}[t]
  \centering
  \input{fig/eval/table-workload}
  \vspace{5pt}
  \captionof{table}{The list of workloads used for evaluation}
  \label{tab:eval-workload}
\end{table}

\PP{Benchmark Applications}
We performed the evaluation with 9 JavaScript serverless
applications as shown in~\autoref{tab:eval-workload}.
We selected the applications from SeBS~\cite{marcin2021sebs}
and Google Sunspider~\cite{sunspider}, which cover a wide
range of applications that receive various secrets as
inputs.

\subsection{Improvement in Function Execution Latency}
\label{ss:eval-latency}
\definecolor{mycolor}{RGB}{200,200,200}

\begin{figure}[t]
  \centering
  \textcolor{mycolor}{
  \boxed{
    \textcolor{black}{
    \;\;\;
    \mbox{\protect\footnotesize{\circled{1}}
      \mbox{$\footnotesize{\cc{Serv}}^{\tiny{\cc{Native}}}$}\xspace}\;\;\;\;\;\;\;\mbox{\protect\footnotesize{\circled{2}}
      \mbox{$\footnotesize{\cc{Serv}}^{\tiny{\cc{CC}}}_{\tiny{\cc{Cold}}}$}\xspace
    }\;\;\;\;\;\;\;\mbox{\protect\footnotesize{\circled{3}}
      \mbox{$\footnotesize{\cc{Serv}}^{\tiny{\cc{CC}}}_{\tiny{\cc{Warm}}}$}\xspace
    }\;\;\;\;\;\;\;\mbox{\protect\footnotesize{\circled{4}}
      \footnotesize{\sys}}
    \;\;\;
    }
    }
    \vspace{-5pt}
  }
  \includegraphics[width=\linewidth]{fig/eval/latency.pdf}
  \caption{Breakdown of function execution latency.
    \cc{Enclave Expand} denotes only the time
    to allocate new EPC pages.
  }
  \label{fig:eval-latencyBreakdown}
\end{figure}
In order to evaluate the latency improvement of \sys, we ran
each benchmark application for 25~times and measured the
average latency as shown in~\autoref{fig:eval-latencyBreakdown}.
\sys (\WC{4}) demonstrated 4.54-6.98$\times$ latency speedup
compared to \modelCcCold (\WC{2}) as it eliminates the
overheads from a new enclave creation (i.e., red part), and
runtime loading (i.e., orange part).
The latency of \enclaveAliasing (which is added instead of
them) was significantly low, ranging from 2.32 to 3.01
milliseconds (i.e., less than 1\% of the entire
latency).
Instead, the latency for allocating additional EPC pages to
load the function instance was the most dominant factor,
taking 27.4-45.6\% of the entire latency.
In addition, \sys showed 1.13-5.28$\times$ higher latency
than \modelCcCold for loading a function instance since it
needs to initiate additional isolation mechanisms (i.e.,
explained in~\autoref{ss:design2-isolation}).

When compared to the conventional serverless computing
(i.e., \modelNative), \sys showed 1.46-3.78$\times$ latency
slowdown.
\modelCcWarm model was the fastest as it pre-loads the
execution environment (e.g., container, enclave, runtime and
the function instance) before receiving the requests.

Given this evaluation, \sys could be further optimized to
pre-allocate the EPC memory.
For example, it would be possible to adaptively pre-allocate
and deallocate the EPC pages considering the latency and
memory usages.
\sys may also adopt request prediction algorithm to
pre-allocate EPC memory, and load the function instance
before receiving the requests.



















\subsection{Improvement of Memory Efficiency}
\label{ss:eval-memory}
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{fig/eval/memory.pdf}
  \caption{Peak EPC memory usage when 64 concurrent requests
    are handled.}
  \label{fig:eval-memory}
\end{figure}

In order to evaluate the memory efficiency of \sys, we
compared the peak EPC memory usage of \sys and \modelCc when
a bunch of requests are received.
In this case, we did not discriminate \modelCcCold and
\modelCcWarm as both need the same amount of EPC memory to
concurrently run the function instances.
For each application, we invoked 64 concurrent requests at
once, and measured the peak EPC memory.
We repeated the experiments three times.


As illustrated in~\autoref{fig:eval-memory}, \sys showed
2.8-5$\times$ lower EPC memory usage compared to \modelCc
when handling 64 concurrent requests.
This is because \modelCc needs to load a new runtime (i.e.,
Gramine library OS~\cite{tsai2017graphene} and
Node.js~\cite{nodejs}) for each request as explained
in~\autoref{sss:motiv-serverless}, while \sys needs to
create only a lightweight V8 Isolate~\cite{v8isolate} on top
of the shared runtime.
In addition, \sys achieves higher memory efficiency as more
requests are concurrently invoked since the more containers
share the same runtime.


On the other hand, \sys uses more memory (i.e., 207MB) than
\modelCc (i.e., 114MB) when handling only one request.
This is because \sys needs additional memory to accommodate
the isolation mechanisms for function instances (i.e., V8
Isolate and file system isolation).










\subsection{Improvement of Throughput}
\label{ss:eval-throughput}

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{fig/eval/throughput-8.pdf}
  \caption{Throughput of each model when handling 8
    requests concurrently.
  }
  \label{fig:eval-throughput-1}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{fig/eval/throughput-64.pdf}
  \caption{Throughput of each model when handling 64
    requests concurrently.
  }
  \label{fig:eval-throughput-2}
\end{figure}

We evaluated the throughput improvement of \sys by invoking
a burst of requests simultaneously and observing the total
time to complete all the requests---i.e., throughput is
computed as the number of requests divided by the completion
time.
To this end, we invoked 8 and 64 requests respectively, for
each model, and measured the average throughput after
repeating the experiments three times.
Especially, we want to note that \sys serves all the
requests with only one enclave, while \modelCc models serve
them with each different enclave.

As a result, \sys exhibited 1.26-3.21$\times$ higher
throughput than \modelCcCold as illustrated
in~\autoref{fig:eval-throughput-1} (i.e., 8 requests invoked
simultaneously), and~\autoref{fig:eval-throughput-2} (i.e.,
64 requests).
Even when compared to \modelNative, \sys showed comparable
performance by decreasing only 5.5-62\% of the native
throughput.
On the other hand, \modelCcWarm showed significantly higher
throughput (i.e., maximum 95$\times$ higher than \sys),
which is attributed to the inherent characteristics of
OpenWhisk---i.e., OpenWhisk is particularly designed to
maximize its performance when used in conjunction with
warm-start mechanisms~\cite{mohan2019agile}.

One thing to note is that the throughput gain of \sys
decreases as the number of requests increases from 8 to 64.
We suspect it is because the SGX driver internally reserves
a lock~\cite{sgxdriver} when allocating the EPC pages, and
the lock contention increases as the number of concurrent
requests increases.
In order to relieve this lock contention, \sys may employ
further optimizations such as batch processing the EPC
allocation requests~\cite{orenbach2017eleos}, or reusing the
allocated EPC pages.
In addition, we want to note that \sys can also create more
enclaves for the same function to maximize the throughput,
while we used only one enclave for this evaluation.

\begin{figure}[t]
  \centering
  \begin{subfigure}{0.48\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{fig/eval/macro-latency.pdf}
    \caption{Latency}
    \label{fig:eval-macro-latency}
  \end{subfigure}
  \begin{subfigure}{0.48\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{fig/eval/macro-memory.pdf}
    \caption{EPC memory usage}
    \label{fig:eval-macro-memory}
  \end{subfigure}
  \caption{
    Latency and EPC memory usage of \modelCcCold,
    \modelCcWarm, and \sys in macro evaluation.
  }
  \label{fig:eval-macro}
\end{figure}

\subsection{Evaluation in Real-world Scenario}
\label{ss:eval-macro}
Finally, we evaluated the performance of \sys assuming the
requests are intermittently arrived as in the real-world
scenario~\cite{shahrad2020serverless,mahmoudi2020performance}.
To this end, we simulated the requests using Poisson
distribution~\cite{rasch1963poisson}, assuming an average
arrival rate of one request per second.
We measured the latency and runtime EPC usage while running
the serverless application (i.e., \cc{dynamic-html}) on each
model.
In this evaluation, \modelCcWarm adopts default warm-start
mechanism of OpenWhisk~\cite{openwhisk} (i.e., reuse-based
mechanism) to reflect the real-world scenario.
In \modelCcWarm, an enclave still remains running after
handling a request and awaits the next request for 30
seconds.

We plotted the latency and runtime EPC usage of each model
as shown in~\autoref{fig:eval-macro}.
As shown in~\autoref{fig:eval-macro-latency}, \sys showed
6.28$\times$ latency speedup over \modelCcCold as already
demonstrated in~\autoref{ss:eval-latency}.
While \modelCcWarm achieved faster latency than \sys on
average, a small number of requests showed huge latency since
it needs to create a new enclave when the number of
concurrent requests are larger than the number of enclaves
already created.
\sys does not suffer from this issue since it has shorter
function startup time by default---i.e., \sys only needs to
alias EPC pages, and loads a new function instance.

Meanwhile, \autoref{fig:eval-macro-memory} shows that \sys
occupies the minimal EPC memory compared to \modelCcCold and
\modelCcWarm.
The interesting observation is that \modelCcCold uses larger
EPC memory than \modelCcWarm, contrary to the common belief
that warm-starts improves the latency at the expense of
memory.
This is because \modelCcWarm reuses already created enclaves
for a new request while \modelCcCold creates a new enclave
for every new request.

\begin{figure}[t]
  \centering
  \begin{subfigure}{0.48\columnwidth}
    \includegraphics[width=\linewidth]{fig/eval/eval-db-latency.pdf}
    \caption{Fork latency}
    \label{fig:motiv-db-latency}
  \end{subfigure}
  \hspace{5pt}
  \begin{subfigure}{0.48\columnwidth}
    \vspace{8pt}
    \includegraphics[width=\linewidth]{fig/eval/eval-db-memory.pdf}
    \caption{Memory Usage}
    \label{fig:motiv-db-memory}
  \end{subfigure}
  \caption{DB comparison}
  \label{fig:motiv-db}
\end{figure}





















==> motivation.tex <==


\section{Problem Statement}
\label{s:motivation}
This paper focuses on performance enhancement of confidential container.
To this end, we first elaborate system model of confidential
container~(\autoref{ss:motiv-system-model}) and its threat
model~(\autoref{ss:motiv-threat-model}).
Then, we analyze the performance issues of previous confidential container
technologies with preliminary
evaluations~(\autoref{ss:motiv-performance-issues}).
Finally, we identify the root cause of these performance limitations and suggest
a solution~(\autoref{ss:motiv-root-cause-and-solution}).

\subsection{System Model}
\label{ss:motiv-system-model}
We assume that cloud customers want to rely on cloud providers to dynamically
manage the resource usage of their applications.
This assumption is based on the common practice in modern cloud computing, such
as function-as-a-service (FaaS)~\cite{} and platform-as-a-service
(PaaS)~\cite{}.
In these cloud computing models, cloud customers delegate the management of
hardware resources to cloud providers.
The cloud providers manage the resource usage of applications dynamically, such
as scaling~\cite{} or resource preemption~\cite{}.
This enables cloud customers to concentrate on application development without
the need to worry about resource management.

Meanwhile, we also assume that cloud customers want to protect sensitive
computations from untrusted cloud environment.
Cloud customers would have a desire to protect their application code (e.g.,
proprietary algorithm) and data (e.g., DNA sequence).
In this scenario, cloud customers do not trust cloud providers, since they might
try unauthorized access to application using full control on privilged system
software. 

Confidential container enables both secure computation on untrusted cloud and
convenient resource management by cloud provider.
Confidential container leverages hardware-based secure enclaves to protect
application data and code from untrusted cloud providers.
In addition, confidential container allows cloud provider to easily manage
hardware resource using container technologies.

\subsection{Threat Model}
\label{ss:motiv-threat-model}
Confidential container's threat model assumes a mutual distrust between cloud
providers and cloud customers who run applications on the cloud. 
Confidential container follows the threat model of confidential computing, where
cloud providers may try to access the application data and code by exploiting
their control over privileged system software. 
In addition, it also adheres to the threat model of containers in cloud
computing, where cloud customers may attempt to breach the system software in
order to gain unauthorized access to other customers' data and code.

Since the main objective of \sys is to improve the performance of
confidential containers, its threat model aligns with that of confidential container. 
The general security limitations of confidential computing are beyond the scope
of this paper.
We do not consider side-channel attacks~\cite{}, which breach the enclave by
monitoring or manipulating the hardware resources (e.g., cache, CPU usage, branch predictor). 
Thus, we assume that cloud providers cannot access the data and code inside the
enclave even though they manage hardware resource.
In addition, addressing the overcharging by cloud providers is orthogonal to our
work~\cite{}.
We also consider denial-of-service attacks as out-of-scope.  

\subsection{Performance Analysis}
\label{ss:motiv-performance-issues}

\subsection{Root Cause and Solution}
\label{ss:motiv-root-cause-and-solution}
\subsubsection{Design Contraint in Confidential Container}
\label{sss:motiv-confidential-container-design}
Confidential container exhibits a design constraint that each container uses own
enclave.
In other words, every process within a container (i.e., a containerized process)
must create a new enclave and run applications within it. 
Specifically, a containerized process initiates the creation of a fresh enclave
and maps the physical enclave region to its virtual address space. 
Then, the containerized process loads data and code into the newly created
enclave and then executes the enclave code.

This design characteristic arises from the traditional approach in confidential
computing, where each enclave is used only by a single process which created it.
This approach does not match well to the design of container.
Since container aims to provide process-level isolation, each container
encapsulates separate processes.
In other words, multiple containers does not share the same process. 
Thus, when the traditional approach of confidential computing is applied to the
container design, a process within each container should use a separate enclave. 

\begin{figure}[t]
  \centering
  \begin{subfigure}{0.60\columnwidth}
    \includegraphics[width=\linewidth]{fig/motiv/motiv-Performance-1.pdf}
    \caption{Startup latency}
    \label{fig:motiv-startup-latency}
  \end{subfigure}
  \hspace{5pt}
  \begin{subfigure}{0.35\columnwidth}
    \vspace{8pt}
    \includegraphics[width=\linewidth]{fig/motiv/motiv-Performance-2.pdf}
    \caption{Data sharing latency}
    \label{fig:motiv-data-sharing-latency}
  \end{subfigure}
  \caption{Performance issues of confidential container\CM{Figure 2b can be changed}}
  \label{fig:motiv-container}
\end{figure}

\subsubsection{Performance Problems}
\label{sss:motiv-performance-analysis}



\subsection{Solution: Sharing Enclave Between Containers}
\label{ss:motiv-solution}






























































































































































































==> rev.tex <==
\gdef\therev{41f90b4}
\gdef\thedate{2024-05-22 20:42:54 +0900}


==> warning.tex <==
\usepackage{silence}
\WarningFilter*{caption}{Unsupported document class}

